IMCRYPTO: An In-Memory Computing Fabric for AES Encryption and Decryption

This paper proposes IMCRYPTO, an in-memory computing (IMC) fabric for accelerating AES encryption and decryption. IMCRYPTO employs a unified structure to implement encryption and decryption in a single hardware architecture, with combined (Inv)SubBytes and (Inv)MixColumns steps. Because of this step-combination, as well as the high parallelism achieved by multiple units of random-access memory (RAM) and random-access/content-addressable memory (RA/CAM) arrays, IMCRYPTO achieves high throughput encryption and decryption without sacrificing area and power consumption. Additionally, due to the integration of a RISC-V core, IMCRYPTO offers programmability and flexibility. IMCRYPTO improves the throughput per area by a minimum (maximum) of 3.3x (223.1x) when compared to previous ASICs/IMC architectures for AES-128 encryption. Projections show added benefit from emerging technologies of up to 5.3x to the area-delay-power product of IMCRYPTO.

==> summary_of_ops.tex <==
\begin{table}[]
    \caption{Summary of Operations \Note{I may need to edit this}}
    \label{tab:operations}
    \centering
    \begin{tabular}{|l|l|}
        \hline
         \textbf{Algorithmic Operation} &  \textbf{Algorithmic/CiM Operation Combination} \\
        \hline
         Fixed point subtract &  Read (Not) + Copy \\
         & Add + copy w/ carry-in = '1' \\ \hline
         Align exponents & Fixed point subtract exponents (for shiftamount) \\ 
         & Write Exponents \\
         & Read + Shift Mantissa (x5) \\ \hline
        Floating point subtract & Align exponents \\
        & Fixed point subtract mantissa \\
        & Read + Shift (x5) to normalize mantissa \\
        & Add + copy to correct exponents \\ \hline
        Floating point summation & Align exponents O(D) \\ 
        & \Note{I need to think about the complexity} \\
        & Accumulate + Shift $O(log_{64} D)$ \\ 
        & Read + Shift \\  \hline
        $2^k$ averaging & Floating point summation \\
                        & Accumulate + Shift \\ 
                        & Shift exponent if necessary \\ \hline
    \end{tabular}
\end{table}{}
